Optimizing Energy-Efficient Braking Trajectories with Anticipatory Road Data for Automated Vehicles

Trajectory planning in automated driving typically focuses on satisfying safety and comfort requirements within the vehicle's onboard sensor range. This paper introduces a method that leverages anticipatory road data, such as speed limits, road slopes, and traffic lights, beyond the local perception range to optimize energy-efficient braking trajectories. For that, coasting, which reduces energy consumption, and active braking are combined to transition from the current vehicle velocity to a lower target velocity at a given distance ahead. Finding the switching instants between the coasting phases and the continuous control for the braking phase is addressed as an optimal trade-off between maximizing coasting periods and minimizing braking effort. The resulting switched optimal control problem is solved by deriving necessary optimality conditions. To facilitate the incorporation of additional feasibility constraints for multi-phase trajectories, a sub-optimal alternative solution based on parametric optimization is proposed. Both methods are compared in simulation.

==> img/architecture.tex <==
%% Creator: Inkscape 1.3 (0e150ed6c4, 2023-07-21), www.inkscape.org
%% PDF/EPS/PS + LaTeX output extension by Johan Engelen, 2010
%% Accompanies image file 'architecture.pdf' (pdf, eps, ps)
%%
%% To include the image in your LaTeX document, write
%%   \input{<filename>.pdf_tex}
%%  instead of
%%   \includegraphics{<filename>.pdf}
%% To scale the image, write
%%   \def\svgwidth{<desired width>}
%%   \input{<filename>.pdf_tex}
%%  instead of
%%   \includegraphics[width=<desired width>]{<filename>.pdf}
%%
%% Images with a different path to the parent latex file can
%% be accessed with the `import' package (which may need to be
%% installed) using
%%   \usepackage{import}
%% in the preamble, and then including the image with
%%   \import{<path to file>}{<filename>.pdf_tex}
%% Alternatively, one can specify
%%   \graphicspath{{<path to file>/}}
%% 
%% For more information, please see info/svg-inkscape on CTAN:
%%   http://tug.ctan.org/tex-archive/info/svg-inkscape
%%
\begingroup%
  \makeatletter%
  \providecommand\color[2][]{%
    \errmessage{(Inkscape) Color is used for the text in Inkscape, but the package 'color.sty' is not loaded}%
    \renewcommand\color[2][]{}%
  }%
  \providecommand\transparent[1]{%
    \errmessage{(Inkscape) Transparency is used (non-zero) for the text in Inkscape, but the package 'transparent.sty' is not loaded}%
    \renewcommand\transparent[1]{}%
  }%
  \providecommand\rotatebox[2]{#2}%
  \newcommand*\fsize{\dimexpr\f@size pt\relax}%
  \newcommand*\lineheight[1]{\fontsize{\fsize}{#1\fsize}\selectfont}%
  \ifx\svgwidth\undefined%
    \setlength{\unitlength}{325.46116866bp}%
    \ifx\svgscale\undefined%
      \relax%
    \else%
      \setlength{\unitlength}{\unitlength * \real{\svgscale}}%
    \fi%
  \else%
    \setlength{\unitlength}{\svgwidth}%
  \fi%
  \global\let\svgwidth\undefined%
  \global\let\svgscale\undefined%
  \makeatother%
  \begin{picture}(1,0.26160068)%
    \lineheight{1}%
    \setlength\tabcolsep{0pt}%
    \put(0.08671493,0.18343512){\color[rgb]{0,0,0}\makebox(0,0)[lt]{\lineheight{1.25}\smash{\begin{tabular}[t]{l}Energy Efficient \\ Trajectory Planning\end{tabular}}}}%
    \put(0.56403935,0.17795312){\color[rgb]{0,0,0}\makebox(0,0)[lt]{\lineheight{1.25}\smash{\begin{tabular}[t]{l}Trajectory Planning \\and Control\end{tabular}}}}%
    \put(0.02165008,0.18935448){\color[rgb]{0,0,0}\makebox(0,0)[lt]{\lineheight{0}\smash{\begin{tabular}[t]{l}$\ve{r}$\end{tabular}}}}%
    \put(0.46498631,0.19019293){\color[rgb]{0,0,0}\makebox(0,0)[lt]{\lineheight{1.5}\smash{\begin{tabular}[t]{l}$\ve{x}_{\mathrm{ref}}$\end{tabular}}}}%
    \put(0.93721874,0.18691483){\color[rgb]{0,0,0}\makebox(0,0)[lt]{\lineheight{1.5}\smash{\begin{tabular}[t]{l}$F_b$\end{tabular}}}}%
    \put(0.27689764,0.02338947){\color[rgb]{0,0,0}\makebox(0,0)[lt]{\lineheight{0}\smash{\begin{tabular}[t]{l}$\ve{x}_{\mathrm{ego}}$, $\ve{p}$\end{tabular}}}}%
    \put(0,0){\includegraphics[width=\unitlength,page=1]{img/architecture1.pdf}}%
  \end{picture}%
\endgroup%


==> img/architecture_vertical.tex <==
%% Creator: Inkscape 1.3 (0e150ed6c4, 2023-07-21), www.inkscape.org
%% PDF/EPS/PS + LaTeX output extension by Johan Engelen, 2010
%% Accompanies image file 'architecture_vertical.pdf' (pdf, eps, ps)
%%
%% To include the image in your LaTeX document, write
%%   \input{<filename>.pdf_tex}
%%  instead of
%%   \includegraphics{<filename>.pdf}
%% To scale the image, write
%%   \def\svgwidth{<desired width>}
%%   \input{<filename>.pdf_tex}
%%  instead of
%%   \includegraphics[width=<desired width>]{<filename>.pdf}
%%
%% Images with a different path to the parent latex file can
%% be accessed with the `import' package (which may need to be
%% installed) using
%%   \usepackage{import}
%% in the preamble, and then including the image with
%%   \import{<path to file>}{<filename>.pdf_tex}
%% Alternatively, one can specify
%%   \graphicspath{{<path to file>/}}
%% 
%% For more information, please see info/svg-inkscape on CTAN:
%%   http://tug.ctan.org/tex-archive/info/svg-inkscape
%%
\begingroup%
  \makeatletter%
  \providecommand\color[2][]{%
    \errmessage{(Inkscape) Color is used for the text in Inkscape, but the package 'color.sty' is not loaded}%
    \renewcommand\color[2][]{}%
  }%
  \providecommand\transparent[1]{%
    \errmessage{(Inkscape) Transparency is used (non-zero) for the text in Inkscape, but the package 'transparent.sty' is not loaded}%
    \renewcommand\transparent[1]{}%
  }%
  \providecommand\rotatebox[2]{#2}%
  \newcommand*\fsize{\dimexpr\f@size pt\relax}%
  \newcommand*\lineheight[1]{\fontsize{\fsize}{#1\fsize}\selectfont}%
  \ifx\svgwidth\undefined%
    \setlength{\unitlength}{205.58086485bp}%
    \ifx\svgscale\undefined%
      \relax%
    \else%
      \setlength{\unitlength}{\unitlength * \real{\svgscale}}%
    \fi%
  \else%
    \setlength{\unitlength}{\svgwidth}%
  \fi%
  \global\let\svgwidth\undefined%
  \global\let\svgscale\undefined%
  \makeatother%
  \begin{picture}(1,0.63044281)%
    \lineheight{1}%
    \setlength\tabcolsep{0pt}%
    \put(0.17195851,0.26162549){\color[rgb]{0,0,0}\makebox(0,0)[lt]{\lineheight{1.25}\smash{\begin{tabular}[t]{l}Trajectory Planning and Control\end{tabular}}}}%
    \put(0.55490802,0.36557044){\color[rgb]{0,0,0}\makebox(0,0)[lt]{\lineheight{1.25}\smash{\begin{tabular}[t]{l}reference trajectory\end{tabular}}}}%
    \put(0.55592721,0.15505182){\color[rgb]{0,0,0}\makebox(0,0)[lt]{\lineheight{1.25}\smash{\begin{tabular}[t]{l}braking command\end{tabular}}}}%
    \put(0.02109556,0.15456352){\color[rgb]{0,0,0}\makebox(0,0)[lt]{\lineheight{1.25}\smash{\begin{tabular}[t]{l}vehicle states\end{tabular}}}}%
    \put(0.55241439,0.58243664){\color[rgb]{0,0,0}\makebox(0,0)[lt]{\lineheight{1.25}\smash{\begin{tabular}[t]{l}road data\end{tabular}}}}%
    \put(0.14385622,0.46558136){\color[rgb]{0,0,0}\makebox(0,0)[lt]{\lineheight{1.25}\smash{\begin{tabular}[t]{l}Energy Efficient Trajectory Planning\end{tabular}}}}%
    \put(0,0){\includegraphics[width=\unitlength,page=1]{img/architecture_vertical1.pdf}}%
    \put(0.45831836,0.04921939){\color[rgb]{0,0,0}\makebox(0,0)[lt]{\lineheight{1.25}\smash{\begin{tabular}[t]{l}Vehicle\end{tabular}}}}%
    \put(0,0){\includegraphics[width=\unitlength,page=2]{img/architecture_vertical1.pdf}}%
  \end{picture}%
\endgroup%


==> img/hybrid_automata.tex <==
%% Creator: Inkscape 1.0.1 (c497b03c, 2020-09-10), www.inkscape.org
%% PDF/EPS/PS + LaTeX output extension by Johan Engelen, 2010
%% Accompanies image file 'hybrid_automata.pdf' (pdf, eps, ps)
%%
%% To include the image in your LaTeX document, write
%%   \input{<filename>.pdf_tex}
%%  instead of
%%   \includegraphics{<filename>.pdf}
%% To scale the image, write
%%   \def\svgwidth{<desired width>}
%%   \input{<filename>.pdf_tex}
%%  instead of
%%   \includegraphics[width=<desired width>]{<filename>.pdf}
%%
%% Images with a different path to the parent latex file can
%% be accessed with the `import' package (which may need to be
%% installed) using
%%   \usepackage{import}
%% in the preamble, and then including the image with
%%   \import{<path to file>}{<filename>.pdf_tex}
%% Alternatively, one can specify
%%   \graphicspath{{<path to file>/}}
%% 
%% For more information, please see info/svg-inkscape on CTAN:
%%   http://tug.ctan.org/tex-archive/info/svg-inkscape
%%
\begingroup%
  \makeatletter%
  \providecommand\color[2][]{%
    \errmessage{(Inkscape) Color is used for the text in Inkscape, but the package 'color.sty' is not loaded}%
    \renewcommand\color[2][]{}%
  }%
  \providecommand\transparent[1]{%
    \errmessage{(Inkscape) Transparency is used (non-zero) for the text in Inkscape, but the package 'transparent.sty' is not loaded}%
    \renewcommand\transparent[1]{}%
  }%
  \providecommand\rotatebox[2]{#2}%
  \newcommand*\fsize{\dimexpr\f@size pt\relax}%
  \newcommand*\lineheight[1]{\fontsize{\fsize}{#1\fsize}\selectfont}%
  \ifx\svgwidth\undefined%
    \setlength{\unitlength}{384.76698768bp}%
    \ifx\svgscale\undefined%
      \relax%
    \else%
      \setlength{\unitlength}{\unitlength * \real{\svgscale}}%
    \fi%
  \else%
    \setlength{\unitlength}{\svgwidth}%
  \fi%
  \global\let\svgwidth\undefined%
  \global\let\svgscale\undefined%
  \makeatother%
  \begin{picture}(1,0.36478467)%
    \lineheight{1}%
    \setlength\tabcolsep{0pt}%
    \put(0.04071063,0.03470795){\color[rgb]{0,0,0}\makebox(0,0)[lt]{\lineheight{1.25}\smash{\begin{tabular}[t]{l}disenganged\end{tabular}}}}%
    \put(0.04031929,0.00412563){\color[rgb]{0,0,0}\makebox(0,0)[lt]{\lineheight{1.25}\smash{\begin{tabular}[t]{l}coasting\end{tabular}}}}%
    \put(0.41849867,0.03828625){\color[rgb]{0,0,0}\makebox(0,0)[lt]{\lineheight{1.25}\smash{\begin{tabular}[t]{l}enganged\end{tabular}}}}%
    \put(0.41810729,0.00770378){\color[rgb]{0,0,0}\makebox(0,0)[lt]{\lineheight{1.25}\smash{\begin{tabular}[t]{l}coasting\end{tabular}}}}%
    \put(0.79095207,0.03676118){\color[rgb]{0,0,0}\makebox(0,0)[lt]{\lineheight{1.25}\smash{\begin{tabular}[t]{l}braking\end{tabular}}}}%
    \put(0.08323253,0.22552052){\color[rgb]{0,0,0}\makebox(0,0)[lt]{\lineheight{1.25}\smash{\begin{tabular}[t]{l}$\dot{\ve{x}}_{q_1}(t)$\end{tabular}}}}%
    \put(0.45239644,0.22552052){\color[rgb]{0,0,0}\makebox(0,0)[lt]{\lineheight{1.25}\smash{\begin{tabular}[t]{l}$\dot{\ve{x}}_{q_2}(t)$\end{tabular}}}}%
    \put(0.74692198,0.22552052){\color[rgb]{0,0,0}\makebox(0,0)[lt]{\lineheight{1.25}\smash{\begin{tabular}[t]{l}$\dot{\ve{x}}_{q_3}(t), u_{q_3}(t)$\end{tabular}}}}%
    \put(0.1243174,0.31019289){\color[rgb]{0,0,0}\makebox(0,0)[lt]{\lineheight{1.25}\smash{\begin{tabular}[t]{l}$q_1$\end{tabular}}}}%
    \put(0.48577687,0.31019289){\color[rgb]{0,0,0}\makebox(0,0)[lt]{\lineheight{1.25}\smash{\begin{tabular}[t]{l}$q_2$\end{tabular}}}}%
    \put(0.84723624,0.31019289){\color[rgb]{0,0,0}\makebox(0,0)[lt]{\lineheight{1.25}\smash{\begin{tabular}[t]{l}$q_3$\end{tabular}}}}%
    \put(0.04814633,0.14739231){\color[rgb]{0,0,0}\makebox(0,0)[lt]{\lineheight{1.25}\smash{\begin{tabular}[t]{l}$t \in [t_0, t_{s_1})$\end{tabular}}}}%
    \put(0.39028706,0.14739231){\color[rgb]{0,0,0}\makebox(0,0)[lt]{\lineheight{1.25}\smash{\begin{tabular}[t]{l}$t \in [t_{s_1}, t_{s_2})$\end{tabular}}}}%
    \put(0.76356491,0.14739231){\color[rgb]{0,0,0}\makebox(0,0)[lt]{\lineheight{1.25}\smash{\begin{tabular}[t]{l}$t \in [t_{s_2},t_f]$\end{tabular}}}}%
    \put(0,0){\includegraphics[width=\unitlength,page=1]{img/hybrid_automata1.pdf}}%
  \end{picture}%
\endgroup%


==> img/opt_trajectories_comparison_time_domain.tex <==
\definecolor{tab_red}{RGB}{240,59,32}
\definecolor{tab_gray}{RGB}{176,176,176}
\definecolor{tab_orange}{RGB}{255,127,14}
\definecolor{tab_green}{RGB}{254,204,92}
\definecolor{dark_gray}{RGB}{127,127,127}
\definecolor{light_gray}{RGB}{204,204,204}
\definecolor{tab_blue}{RGB}{253,141,60}

\usetikzlibrary{math} %needed tikz library

\tikzmath{\ts1 = 9.27; \ts2 = 12.62; \tf = 18.21;}
%t_s1 = 9.04656095425038
%t_s2 = 13.0637480036
%t_f = 18.3463120894715


\begin{center}
\begin{tabular}{r}
\begin{tikzpicture}
\begin{axis}[
	width = 0.47\textwidth,
	height = 3.3cm,
	ylabel = {$s_q$ [m]},
	xmin = 0,
	ymin = 0,
	xmax = 13.8,
	grid = major,
	grid style = {dotted, black},
	legend style = {
		draw = none,
		font = \small,
		at = {(0.5, 1.05)},
		anchor = south,
		},
	ytick distance = 250,
	legend columns=3,
	%extra x ticks = {\ts1, \ts2, \tf},
	%extra x tick style = {
				%major grid style = {black, dashed, thick},
	%},
	%extra x tick labels= {,,,},
	]
	\addplot[tab_green, line width=3.8pt, opacity=0.4] table [col sep=comma, x=t, y = s] {img/data/s_q1_t_im.csv};
	\addlegendentry{$q_1$, i.m.};
	
	\addplot[tab_blue, line width=3.8pt, opacity=0.4] table [col sep=comma, x=t, y = s] {img/data/s_q2_t_im.csv};
	\addlegendentry{$q_2$, i.m.};
	
	\addplot[tab_red, line width=3.8pt, opacity=0.4] table [col sep=comma, x=t, y = s] {img/data/s_q3_t_im.csv};
	\addlegendentry{$q_3$, i.m.};
	
	\addplot[tab_green, line width=1.5pt, densely dashed] table [col sep=comma, x=t, y = s] {img/data/s_q1_t_dm.csv};
	\addlegendentry{$q_1$, d.m.};
	
	\addplot[tab_blue, line width=1.5pt, densely dashed] table [col sep=comma, x=t, y = s] {img/data/s_q2_t_dm.csv};
	\addlegendentry{$q_2$, d.m.};
	
	\addplot[tab_red, line width=1.5pt, densely dashed] table [col sep=comma, x=t, y = s] {img/data/s_q3_t_dm.csv};
	\addlegendentry{$q_3$, d.m.};
	
	\addplot[black, line width=0.8pt, dashed] table [col sep=comma, x=t_f, y=s_f] {img/data/s_f.csv} [yshift = -6pt] node [pos=0.03] {$s_f$};
	
\end{axis}
\end{tikzpicture}
\\

\begin{tikzpicture}
\begin{axis}[
	width = 0.47\textwidth,
	height = 3.3cm,
	ylabel = {$v_q$ [km/h]},
	xmin = 0,
	xmax = 13.8,
	grid = major,
	grid style = {dotted, black},
	legend style = {
		font = \small,
		at = {(0.67, 0.55)},
		anchor = south west,
		},
	ytick distance = {25},
	%extra x ticks = {\ts1, \ts2, \tf},
	%extra x tick style = {
	%			major grid style = {black, dashed, thick},
	%},
	%extra x tick labels= {,,,},
	]
	\addplot[tab_green, line width=3.8pt, opacity=0.4] table [col sep=comma, x=t, y = v] {img/data/v_q1_t_im.csv};
	
	\addplot[tab_blue, line width=3.8pt, opacity=0.4] table [col sep=comma, x=t, y = v] {img/data/v_q2_t_im.csv};
	
	\addplot[tab_red, line width=3.8pt, opacity=0.4] table [col sep=comma, x=t, y = v] {img/data/v_q3_t_im.csv};
	
	\addplot[tab_green, line width=1.5pt, densely dashed] table [col sep=comma, x=t, y = v] {img/data/v_q1_t_dm.csv};
	
	\addplot[tab_blue, line width=1.5pt, densely dashed] table [col sep=comma, x=t, y = v] {img/data/v_q2_t_dm.csv};
	
	\addplot[tab_red, line width=1.5pt, densely dashed] table [col sep=comma, x=t, y = v] {img/data/v_q3_t_dm.csv};
	
	\addplot[black, line width=0.8pt, dashed] table [col sep=comma, x=t_f, y=v_f] {img/data/v_f.csv}[yshift = 6pt] node [pos=0.03] {$v_f$};
	
\end{axis}
\end{tikzpicture}
\\

\begin{tikzpicture}
\begin{axis}[
	width = 0.47\textwidth,
	height = 3.3cm,
	xlabel = {$t$ [s]},
	ylabel = {$u_q$ [m/$\text{s}^2$]},
	xmin = 0,
	xmax = 13.8,
	grid = major,
	grid style = {dotted, black},
	%extra x ticks = {\ts1, \ts2, \tf},
	%extra x tick style = {
	%			major grid style = {black, dashed, thick},
	%			tick align = outside,
	%			ticklabel style = {yshift = 22pt, xshift=-8pt},
	%},
	%extra x tick labels = {$t_{s_1}$, $t_{s_2}$, $t_f$},
	]
	\addplot[tab_green, line width=3.8pt, opacity=0.4] table [col sep=comma, x=t, y = u] {img/data/u_q1_t_im.csv};
	
	\addplot[tab_blue, line width=3.8pt, opacity=0.4] table [col sep=comma, x=t, y = u] {img/data/u_q2_t_im.csv};
	
	\addplot[tab_red, line width=3.8pt, opacity=0.4] table [col sep=comma, x=t, y = u] {img/data/u_q3_t_im.csv};
	
	\addplot[tab_green, line width=1.5pt, densely dashed] table [col sep=comma, x=t, y = u] {img/data/u_q1_t_dm.csv};
	
	\addplot[tab_blue, line width=1.5pt, densely dashed] table [col sep=comma, x=t, y = u] {img/data/u_q2_t_dm.csv};
	
	\addplot[tab_red, line width=1.5pt, densely dashed] table [col sep=comma, x=t, y = u] {img/data/u_q3_t_dm.csv};
	
\end{axis}

\end{tikzpicture}

\end{tabular}

\end{center}


==> img/switched_system.tex <==
%% Creator: Inkscape 1.3 (0e150ed6c4, 2023-07-21), www.inkscape.org
%% PDF/EPS/PS + LaTeX output extension by Johan Engelen, 2010
%% Accompanies image file 'switched_system.pdf' (pdf, eps, ps)
%%
%% To include the image in your LaTeX document, write
%%   \input{<filename>.pdf_tex}
%%  instead of
%%   \includegraphics{<filename>.pdf}
%% To scale the image, write
%%   \def\svgwidth{<desired width>}
%%   \input{<filename>.pdf_tex}
%%  instead of
%%   \includegraphics[width=<desired width>]{<filename>.pdf}
%%
%% Images with a different path to the parent latex file can
%% be accessed with the `import' package (which may need to be
%% installed) using
%%   \usepackage{import}
%% in the preamble, and then including the image with
%%   \import{<path to file>}{<filename>.pdf_tex}
%% Alternatively, one can specify
%%   \graphicspath{{<path to file>/}}
%% 
%% For more information, please see info/svg-inkscape on CTAN:
%%   http://tug.ctan.org/tex-archive/info/svg-inkscape
%%
\begingroup%
  \makeatletter%
  \providecommand\color[2][]{%
    \errmessage{(Inkscape) Color is used for the text in Inkscape, but the package 'color.sty' is not loaded}%
    \renewcommand\color[2][]{}%
  }%
  \providecommand\transparent[1]{%
    \errmessage{(Inkscape) Transparency is used (non-zero) for the text in Inkscape, but the package 'transparent.sty' is not loaded}%
    \renewcommand\transparent[1]{}%
  }%
  \providecommand\rotatebox[2]{#2}%
  \newcommand*\fsize{\dimexpr\f@size pt\relax}%
  \newcommand*\lineheight[1]{\fontsize{\fsize}{#1\fsize}\selectfont}%
  \ifx\svgwidth\undefined%
    \setlength{\unitlength}{497.04051581bp}%
    \ifx\svgscale\undefined%
      \relax%
    \else%
      \setlength{\unitlength}{\unitlength * \real{\svgscale}}%
    \fi%
  \else%
    \setlength{\unitlength}{\svgwidth}%
  \fi%
  \global\let\svgwidth\undefined%
  \global\let\svgscale\undefined%
  \makeatother%
  \begin{picture}(1,0.37810371)%
    \lineheight{1}%
    \setlength\tabcolsep{0pt}%
    \put(0,0){\includegraphics[width=\unitlength,page=1]{img/switched_system1.pdf}}%
    \put(0.12542164,0.32797802){\color[rgb]{0,0,0}\makebox(0,0)[lt]{\lineheight{1.5}\smash{\begin{tabular}[t]{l}$q_1$\end{tabular}}}}%
    \put(0.47541683,0.3219423){\color[rgb]{0,0,0}\makebox(0,0)[lt]{\lineheight{1.5}\smash{\begin{tabular}[t]{l}$q_2$\end{tabular}}}}%
    \put(0.82541179,0.31892443){\color[rgb]{0,0,0}\makebox(0,0)[lt]{\lineheight{1.5}\smash{\begin{tabular}[t]{l}$q_3$\end{tabular}}}}%
    \put(0.09813282,0.21953457){\color[rgb]{0,0,0}\makebox(0,0)[lt]{\lineheight{1.5}\smash{\begin{tabular}[t]{l}$\dot{\ve{x}}_{q_1}(t)$\end{tabular}}}}%
    \put(0.43658105,0.21953457){\color[rgb]{0,0,0}\makebox(0,0)[lt]{\lineheight{1.5}\smash{\begin{tabular}[t]{l}$\dot{\ve{x}}_{q_2}(t)$\end{tabular}}}}%
    \put(0.73290144,0.21953457){\color[rgb]{0,0,0}\makebox(0,0)[lt]{\lineheight{1.5}\smash{\begin{tabular}[t]{l}$\dot{\ve{x}}_{q_3}(t), u_{q_3}(t)$\end{tabular}}}}%
    \put(0.06071523,0.14238032){\color[rgb]{0,0,0}\makebox(0,0)[lt]{\lineheight{1.5}\smash{\begin{tabular}[t]{l}$t \in \left[t_0, t_{s_1} \right)$\end{tabular}}}}%
    \put(0.39768734,0.14238032){\color[rgb]{0,0,0}\makebox(0,0)[lt]{\lineheight{1.5}\smash{\begin{tabular}[t]{l}$t \in \left[t_{s_1}, t_{s_2} \right)$\end{tabular}}}}%
    \put(0.7411576,0.14238032){\color[rgb]{0,0,0}\makebox(0,0)[lt]{\lineheight{1.5}\smash{\begin{tabular}[t]{l}$t \in \left[t_{s_2}, t_f \right]$\end{tabular}}}}%
    \put(0.05182442,0.03211201){\color[rgb]{0,0,0}\makebox(0,0)[lt]{\lineheight{1.5}\smash{\begin{tabular}[t]{l}disengaged \\coasting\end{tabular}}}}%
    \put(0.43154181,0.03211201){\color[rgb]{0,0,0}\makebox(0,0)[lt]{\lineheight{1.5}\smash{\begin{tabular}[t]{l}engaged \\coasting\end{tabular}}}}%
    \put(0.78759078,0.03233304){\color[rgb]{0,0,0}\makebox(0,0)[lt]{\lineheight{1.5}\smash{\begin{tabular}[t]{l}braking\end{tabular}}}}%
  \end{picture}%
\endgroup%

